Automatic Generation of Grover Quantum Oracles for Arbitrary Data Structures

The steadily growing research interest in quantum computing - together with the accompanying technological advances in the realization of quantum hardware - fuels the development of meaningful real-world applications, as well as implementations for well-known quantum algorithms. One of the most prominent examples till today is Grover's algorithm, which can be used for efficient search in unstructured databases. Quantum oracles that are frequently masked as black boxes play an important role in Grover's algorithm. Hence, the automatic generation of oracles is of paramount importance. Moreover, the automatic generation of the corresponding circuits for a Grover quantum oracle is deeply linked to the synthesis of reversible quantum logic, which - despite numerous advances in the field - still remains a challenge till today in terms of synthesizing efficient and scalable circuits for complex boolean functions. In this paper, we present a flexible method for automatically encoding unstructured databases into oracles, which can then be efficiently searched with Grover's algorithm. Furthermore, we develop a tailor-made method for quantum logic synthesis, which vastly improves circuit complexity over other current approaches. Finally, we present another logic synthesis method that considers the requirements of scaling onto real world backends. We compare our method with other approaches through evaluating the oracle generation for random databases and analyzing the resulting circuit complexities using various metrics.

==> sections/summary_backup.tex <==
\section{Summary}
\label{summary}

The current paper provides a first successful attempt for enabling the convenient and efficient utilization of
Grover's search algorithm capabilities over traditional function/procedure APIs (e.g.
\textit{int grover(int [] list\_to\_search\_in, int value\_to\_search\_for)}). The motivation
for this research is based on observations in our previous work \cite{GheorghePop2021}, in which
the issues of constructing oracles for Grover database searches was discussed from a user perspective.
Indeed, the only way to make quantum computing comercially viable is to provide accessible 
APIs and interfaces for programers and end users to integrate quantum algorithms in their
services and applications.

With regard to Grover's algorithm, such APIs require for the automatic generation
of the black box quantum oracles, which contain the database and the element to
search for in this database. In this context, our current paper provides a methodology 
for automatically generating such quantum oracles for arbitrary databases. The generation
consists of two main parts: 1) Mapping the database entries to binary hash values and 2)
using quantum logical synthesis to create the corresponding oracle functions based 
on automatically prepared truth tables. The first step is easily realized through
the utilization of state-of-the-art hash functions, whilst the second step requires different 
methods for quantum logical synthesis to be applied. In this regard, one of the main contributions
of this paper is given by application methods such as the Gray synthesis to the problem of Grover quantum
oracle generation. Furthermore, we present new methods for the fault-tolerant implementation
of Grover oracle function - i.e. \textit{Phase Tolerant Synthesis} and a synthesis method respecting the requirements of fault tolerant implementations. The novelty of these two methods is constituted 
by the improvements in the CNOT gate counts as well as in the resilience with respect
to noise in the qubits during the computation process. Both methods proposed within
our research work and presented here prove to be more effective than the standard methods for
quantum logical synthesis within the task of Grover oracle generation. These observations 
stem from a number of benchmarking evaluations that were conducted in the course of our research and 
presented in the current paper.

To summarize: this paper outlines a clear procedure for making the potentials of the powerful quantum algorithm by Grover available to programmers and end users for integration in
everyday ICT-systems (e.g. online shops, telecommunication management systems, database search engines,
web analytic systems ...). The methodology proposed in this paper generates the belonging quantum
oracles automatically, thereby utilizing and leading to innovative methods for quantum logic synthesis.
The computational complexity of the methodology is in general higher than the one of Grover's
algorithm. However, our future research works aims at optimizing this complexity through different 
heuristics, machine learning techniques and optimizations on the proposed approach. By continuously achieving such
gradual improvements, one can see a clear path to a full-scale introduction and application of 
quantum algorithms based on oracles in current development processes and system architectures.

